E-Branchformer: Branchformer with Enhanced merging for speech recognition

Conformer, combining convolution and self-attention sequentially to capture both local and global information, has shown remarkable performance and is currently regarded as the state-of-the-art for automatic speech recognition (ASR). Several other studies have explored integrating convolution and self-attention but they have not managed to match Conformer's performance. The recently introduced Branchformer achieves comparable performance to Conformer by using dedicated branches of convolution and self-attention and merging local and global context from each branch. In this paper, we propose E-Branchformer, which enhances Branchformer by applying an effective merging method and stacking additional point-wise modules. E-Branchformer sets new state-of-the-art word error rates (WERs) 1.81% and 3.65% on LibriSpeech test-clean and test-other sets without using any external training data.

==> tables/others.tex <==
\begin{table}[th]
\caption{Comparison of word error rates (WER) and the computational complexity (MACs) depending on whether FFN or macaron-style FFN is applied or not. We do not change the original Branchformer block, and no external LM is used for evaluations.}
\label{table:ffn}
\begin{center}
\resizebox{\linewidth}{!}
{
\begin{tabular}{lccccccc}
\hline
\multirow{2}{*}{Model} & \# of & Enc. & MACs & dev & dev & test & test \\
 & layers & Params (M) & (G) & clean & other & clean & other \\
\hline\hline
% BranchFormer & 24 & 142.42 & 2.1 & 5.0 & 2.2 & 5.0 \\
BranchFormer & 25 & 113.8 & 43.7 & 2.01 & 4.99 & 2.25 & 4.83 \\
\tabindent{+ FFN} & 17 & 115.4 & \textbf{42.6} & 1.98 & 4.83 & 2.18 & 4.87 \\
\tabindent{+ FFN-mac} & 13 & 117.3 & \textbf{42.3} & 1.97 & 4.74 & 2.26 & 4.74 \\
\tabindent{+ FFN-mac-n} & 17 & 115.5 & \textbf{42.6} & 1.97 & 4.78 & 2.10 & 4.79 \\
\tabindent{+ FFN-mac} & 17 & 151.1 & 51.5 & 2.00 & 4.75 & 2.15 & 4.47 \\
\hline
\end{tabular}
}
\end{center}
\end{table}
